It's Like Python But: Towards Supporting Transfer of Programming Language Knowledge

Expertise in programming traditionally assumes a binary novice-expert divide. Learning resources typically target programmers who are learning programming for the first time, or expert programmers for that language. An underrepresented, yet important group of programmers are those that are experienced in one programming language, but desire to author code in a different language. For this scenario, we postulate that an effective form of feedback is presented as a transfer from concepts in the first language to the second. Current programming environments do not support this form of feedback. In this study, we apply the theory of learning transfer to teach a language that programmers are less familiar with--such as R--in terms of a programming language they already know--such as Python. We investigate learning transfer using a new tool called Transfer Tutor that presents explanations for R code in terms of the equivalent Python code. Our study found that participants leveraged learning transfer as a cognitive strategy, even when unprompted. Participants found Transfer Tutor to be useful across a number of affordances like stepping through and highlighting facts that may have been missed or misunderstood. However, participants were reluctant to accept facts without code execution or sometimes had difficulty reading explanations that are verbose or complex. These results provide guidance for future designs and research directions that can support learning transfer when learning new programming languages.

==> tables/explanations.tex <==
\begin{table}
\caption{Learning Message Descriptions\label{tbl:methodology:explanations}}
\begin{threeparttable}
\begin{tabularx}{\columnwidth}{llX}
  \toprule
  % & \multicolumn{3}{c}{\textbf{Question Count}\tnote{2}}\\
  % \cmidrule(lr){2-4}
  \textbf{Tag} & \textbf{Method} & \textbf{Programming Language Explanations}\\
  \midrule
  L1 & \nontransfer & \\
  \addlinespace
     & \transfer & Watch out! The inner \texttt{[]} cannot be used to select a list of columns in R. The [[ syntax is allowed in R but it can only be used to select one column. \\
  \midrule
  L2 & \nontransfer & \texttt{cannot find symbol}\\
     &         & \texttt{symbol:   variable varnam}\\
     &         & \texttt{location: class Foo}\\
  \addlinespace
     & \transfer & The \texttt{[]} syntax can be used in R to subset data frames.\\
  \midrule
  L3 & \nontransfer & You can read csv files with: \texttt{df <- read.csv('Questions.csv')}\\
  \addlinespace
     & \transfer & R variable names can consist of alphanumerics and dot (\texttt{.}) and underscore (\texttt{\_}) so it's not safe to assume the dot signifies method dispatch. So 'read' here is not really an Object as you might guess coming from a language like Python.\\
  \midrule
  L4 & \nontransfer & You can use the \texttt{[} syntax to select columns from the data frame.\\
  \addlinespace    
     & \transfer & Using the [, x] syntax to subset requires specifying both a row and column selection of the dataframe. You still need a comma here but you may leave the row side to be empty to signify that you want all rows. Likewise, if selecting all columns you can leave the column side empty.\todo{Might want to make this more explicit to Python. R allows subsetting like in Python. But...}\\
  \midrule
  L5 & \nontransfer & \texttt{Illegal static declaration in inner class A.B. Modifier 'static' is only allowed in constant variable declarations.}\\
  \addlinespace
     & \transfer & \texttt{This static variable declaration is invalid, because it is not final, but is enclosed in an inner class, "B".}\\
  \bottomrule
  
\end{tabularx}
\end{threeparttable}
\end{table}

==> tables/survey-results.tex <==
\newcommand{\taskbox}[1]{%
\begin{tikzpicture}[xscale=0.05,yscale=0.1,baseline=(current bounding box.south)]    
  \draw[fill=white] (0,0) rectangle (10, 1.5);
  \draw[fill=black] (0,0) rectangle ($(#1/10, 1.5)$);
\end{tikzpicture}
}

\newcommand{\taskboxsig}[1]{%
\begin{tikzpicture}[xscale=0.05,yscale=0.1,baseline=(current bounding box.south)]    
  \draw[fill=white] (0,0) rectangle (10, 1.5);
  \draw[fill=black!30!green] (0,0) rectangle ($(#1/10, 1.5)$);
\end{tikzpicture}
}

\begin{table}
\begin{threeparttable}
\caption{Non-transfer and Transfer Explanations Preferences\label{tbl:results:transfer}}
\begin{tabularx}{.75\columnwidth}{lXllll}
  \toprule
  & & \multicolumn{2}{c}{\textbf{Non-transfer}} & \multicolumn{2}{c}{\textbf{Transfer}}\\
  \cmidrule(lr){3-4} \cmidrule(lr){5-6}
  \textbf{Tag} & \emph{p}\tnote{1} & n & \% & n & \%\\
  \midrule
  L1 & .001* & 2  &\taskbox{3} 3\%   & 66 &\taskboxsig{97} 97\%\\
  L2 & .014* & 20 &\taskbox{29} 29\% & 48 &\taskboxsig{71} 71\%\\
  L3 & .037* & 46 &\taskboxsig{68} 68\% & 22 &\taskbox{32} 32\%\\
  L4 & .014* & 20 &\taskbox{29} 29\% & 48 &\taskboxsig{70} 70\%\\
  L5 & .732 & 36 &\taskbox{53} 53\% & 32 &\taskbox{47} 47\%\\
  \bottomrule
\end{tabularx}
\begin{tablenotes}
\item[1] * indicates a statistically significant result.
\end{tablenotes}
\end{threeparttable}
\end{table}
